Automated Attack Synthesis by Extracting Finite State Machines from Protocol Specification Documents

Automated attack discovery techniques, such as attacker synthesis or model-based fuzzing, provide powerful ways to ensure network protocols operate correctly and securely. Such techniques, in general, require a formal representation of the protocol, often in the form of a finite state machine (FSM). Unfortunately, many protocols are only described in English prose, and implementing even a simple network protocol as an FSM is time-consuming and prone to subtle logical errors. Automatically extracting protocol FSMs from documentation can significantly contribute to increased use of these techniques and result in more robust and secure protocol implementations. In this work we focus on attacker synthesis as a representative technique for protocol security, and on RFCs as a representative format for protocol prose description. Unlike other works that rely on rule-based approaches or use off-the-shelf NLP tools directly, we suggest a data-driven approach for extracting FSMs from RFC documents. Specifically, we use a hybrid approach consisting of three key steps: (1) large-scale word-representation learning for technical language, (2) focused zero-shot learning for mapping protocol text to a protocol-independent information language, and (3) rule-based mapping from protocol-independent information to a specific protocol FSM. We show the generalizability of our FSM extraction by using the RFCs for six different protocols: BGPv4, DCCP, LTP, PPTP, SCTP and TCP. We demonstrate how automated extraction of an FSM from an RFC can be applied to the synthesis of attacks, with TCP and DCCP as case-studies. Our approach shows that it is possible to automate attacker synthesis against protocols by using textual specifications such as RFCs.

==> fordiscussion.tex <==
,
	although it is sensitive to the choice of properties.
A good property should be \emph{broad} in that it relates to behaviors in many
different parts of the protocol, but also \emph{robust} in that it is not easily violated
or made vacuous by small bugs in the protocol \fsm.
In lieu of such broad and robust properties, an alternative approach is to write properties that
each relate precisely to different non-overlapping parts of the protocol \fsm,
	so that the conjunction is broad and the disjunction is robust.
From an attacker synthesis perspective, our pipeline
	could be improved using some mechanism for \emph{patching}
	broken or partial \program s.
This could be done formally 
	(as in~\cite{alur2017automatic}), 
or heuristically.


==> fsm-figures/q.tex <==
\relax 
\@setckpt{dccp/linear/linear.dccp}{
\setcounter{page}{5}
\setcounter{equation}{0}
\setcounter{enumi}{5}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{3}
\setcounter{table}{0}
\setcounter{parentequation}{0}
}

